Neural Computed Tomography

Motion during acquisition of a set of projections can lead to significant motion artifacts in computed tomography reconstructions despite fast acquisition of individual views. In cases such as cardiac imaging, motion may be unavoidable and evaluating motion may be of clinical interest. Reconstructing images with reduced motion artifacts has typically been achieved by developing systems with faster gantry rotation or using algorithms which measure and/or estimate the displacements. However, these approaches have had limited success due to both physical constraints as well as the challenge of estimating/measuring non-rigid, temporally varying, and patient-specific motions. We propose a novel reconstruction framework, NeuralCT, to generate time-resolved images free from motion artifacts. Our approaches utilizes a neural implicit approach and does not require estimation or modeling of the underlying motion. Instead, boundaries are represented using a signed distance metric and neural implicit framework. We utilize `analysis-by-synthesis' to identify a solution consistent with the acquired sinogram as well as spatial and temporal consistency constraints. We illustrate the utility of NeuralCT in three progressively more complex scenarios: translation of a small circle, heartbeat-like change in an ellipse's diameter, and complex topological deformation. Without hyperparameter tuning or change to the architecture, NeuralCT provides high quality image reconstruction for all three motions, as compared to filtered backprojection, using mean-square-error and Dice metrics.

==> old_stuff.tex <==

\newpage

\newpage


Figure:
Panel A) Plot of the Metric above vs speed (x-axis) for FBP (solid) vs NeuralCT (dashed) for different offsets (colors)
Panel B) Visualization of "cylinders" above wit 3 experiments at a single speed/offset


\subsection{How does this work?} 
Series of ablation experiments on dots showing contributors to accuracy
- TV 2D sweep of spatial vs temporal
- Fourier coefficients 
- Eikonal constraint change

- Siren as MLP vs regular MLP (skip for now - not the focus, to some extent expected and complicated story)
- Super resolution (futre result)


\newpage
\section{Extra Experiments: For future papers}
\label{sec:extra_experiments}
\subsection{Periodic motion: Heart imaging}
Compare is 1 cycle to 1 second imaging
As it gets faster, 1 cycle falls apart but 1 second imaging shows we can seamlessly incorporate multiple views and make a great image
- Need phase information

Temporal projections thru the object to show a smooth transition that matches the analytic answer
Multiple gantry rotations to observe a moving object

Figure 1: Make a temporal slice at (x=0,y,t) which shows the beating as a 1D displacement. One row is the truth, 2nd row is the FBP with step artifacts and 3rd is neural CT. Make the movie aperiodic and highlight fast regions. Like elliots grant


\subsection{Generalizability of approach: Evaluation of a range of motion types and multiple intensities} 

Topology Change Movie: A to B to C
Use the A to B to C movie to show ability to reconstruct not just dots but complex motion

Can also show Figure 8 motion?
We will keep UCSD example for talks

Two objects moving/beating

\subsection{Extension to Dual-Source and Prolonged Acquisitions}
Figure 3: How does having 2 spins of a cyclic motion help

Figure 4: How does having 2 detectors complement this method


% \begin{figure}[!t]
% \centerline{\includegraphics[width=\columnwidth]{fig1.png}}
% \caption{Magnetization as a function of applied field.
% It is good practice to explain the significance of the figure in the caption.}
% \label{fig1}
% \end{figure}


\newpage

\section{Old Text}


This has typically led to the use of constraints on the motion field (e.g. rigid body framework or optical flow penalization of divergence of non-rigid motion), regularization (e.g. TV constraint on intensity, divergence of non-rigid motion field) or observations.

requires estimating motion in regions with little to no intensity change. 


\subsection{Velocity network}
Motion has been solved for using a variety of motion models ranging from simple translations to complex non-rigid deformations. 
In our approach, the SDFs (and their evolution via band-limited Fourier features) are used to restrict the evolution of physical object boundaries to be consistent with physiologically realistic motions.  
For example, use of HR to control rate of evolution.

\begin{itemize}
    \item Motion artifacts are a significant problem in CT scanning and occur in the reconstructed image due to motion during the data acquisition.
    \item While individual projections are acquired incredibly quickly, a complete set of data takes some time (~0.5 seconds) to be acquired. 
    \item Reconstruction approaches such as FBP assume data is acquired simultaneously and therefore changes in the object position lead to inconsistencies that result in artifacts. 
\end{itemize}

\vspace{1cm}
\begin{itemize}
    
    \item Another way of framing the FBP reconstruction is that it aims to represents data acquired of a moving object not as a temporally-evolving image sequence (movie) but rather as a single image frame. 
    \item To this end, clinical applications try to identify relatively stationary periods of motion (imaging the heart during diastasis or end-systole for near-stationary coronary artery images).
    \item However, even small residual motions remain problematic (cite FC coronary motion paper)
 \end{itemize}

\vspace{1cm}
\begin{itemize}
    \item Representing the acquired data as a movie would significantly increase the complexity of the problem.
    \item Specific problems: 1) computational load of solving for a movie increases (e.g. solving for N volumes simultaneously), 2) this increases the number of unknowns (significantly ill-posed problem).
    \item This leads to solutions that would either be computational intractable or cannot be sufficiently regularized.
    \item One cause of these limitations is that the reconstruction representation is inefficient. 
    \item First, the image is represented as an array of voxels with intensity (which become time-varying intensity voxels in the case of a movie). This results in an already computational demanding 3D volume of voxels further scaling linearly with the temporal dimension. 
    \item Further, medical CT imaging aims to represent physical objects where attenuation values are fairly homogeneous in intensity with sharp boundaries. In the case of moving objects, the artifacts arise from (and clinical interest lies in) the location/motion of these boundaries.
    \item As a result, the voxel array (and prior dimensionality reduction techniques like a wavelet transform or Fourier) are ill suited for the task.
\end{itemize}

\vspace{1cm}
\begin{itemize}    
    \item Two innovations: Implicit Representation (spatial and temporal data) and SDF
    \item Two by two array of representations: Voxels vs Implicit     and Intensity vs SDF
    \item SDFs have been used to represent anatomy but we are the first to do it for CT reconstruction
    \item MLPs/implicit have been used to represent medical images (intensity) but not SDFs.
    \item However, nobody has combined SDF with implicit spatiotemporal representation at all? for image recon? for CT?
    \item Developed the pipeline to do this
    
    \item We provide the first way to take data acquired on a scanner (at realistic time and length scales) and reconstruct moving objects at relevant length/time scales.

\end{itemize}    

\vspace{1cm}
\begin{itemize}
    \item while the location of boundaries is of interest for movies, the voxel array represents the entire volume with equal concern.
    
    \item Issues with existing voxel based representation
    \item how to put adequate regularizations to better constrain the problem?
    
    \item object aware representation of anatomy
    \item physically based modelling of object dynamics
    
    \item toy example?
\end{itemize}



\subsection{Initialization}
Definition of Objects with Filtered Backprojection with GMM to identify initial "classes"
Given eikonal constraint, we need sensible gradients so we initialize. 
If we don't it fails. But by no means is this the only way to do it or even the best.

\subsection{Initial Training}
Losses: TV in time, space and iconal.
May or may not have ablations (like the Neural Mesh Flow paper)

\subsection{Refinement}
Regularization with TV
May or may not have ablations (like the Neural Mesh Flow paper)


Figure 3: Velocity network 
Figure 4: Visualize stages of Neural CT (as an example)


Figure A: Toy example idea 1
1) If we have sparse sinogram data, do we do a better job at reconstructing with an SDF?
Object takes a particular form - representation is an SDF that becomes occupancy and then render
Smooth boundaries would cause SDF to fail
Inverse: sharp boundaries
Object is well described by uniform inside intensity vs outer intensity?

Smoothly moves in time

Figure B: Toy example idea 2
1) We have a circle/square that goes from small diameter to large and we can show its diameter via a i(x=0,y,t) slice
2) With a series of FBP recons (or any voxel based recon) makes no boundary distinctions so the the boundary is correct and incorrect as a function of CT rotation
3) Only image series that is consistent with sinogram data and is a moving topological object
4) However, the NeuralCT approach learns the more obvious manifold F which is a smoothly varying instead of learning individual slices at each time point.
5) Show FBP, CS+TV, and NeuralCT

\section{Discussion}

The performance degrades at the start/end of movie. Show the degradation performance as a function of time in movie. 


\subsection{Discussion Point 1: Tradeoff of our design}
By construction, implicit representation is object-centric. 
In this setting, this eliminates intensity variations (i.e. texture) and significantly simplifies our representation which we hypothesize facilitates tracking of boundary motion.
Further, we believe this can complement intensity (texture)-based efforts (described above) since estimates of boundary position can serve as useful constraints for intensity-based algorithms.
% \begin{table}
% \caption{Units for Magnetic Properties}
% \label{table}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{|p{25pt}|p{75pt}|p{115pt}|}
% \hline
% Symbol& 
% Quantity& 
% Conversion from Gaussian and \par CGS EMU to SI $^{\mathrm{a}}$ \\
% \hline
% $\Phi $& 
% magnetic flux& 
% 1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V$\cdot $s \\
% $B$& 
% magnetic flux density, \par magnetic induction& 
% 1 G $\to  10^{-4}$ T $= 10^{-4}$ Wb/m$^{2}$ \\
% $H$& 
% magnetic field strength& 
% 1 Oe $\to  10^{3}/(4\pi )$ A/m \\
% $m$& 
% magnetic moment& 
% 1 erg/G $=$ 1 emu \par $\to 10^{-3}$ A$\cdot $m$^{2} = 10^{-3}$ J/T \\
% $M$& 
% magnetization& 
% 1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 10^{3}$ A/m \\
% 4$\pi M$& 
% magnetization& 
% 1 G $\to  10^{3}/(4\pi )$ A/m \\
% $\sigma $& 
% specific magnetization& 
% 1 erg/(G$\cdot $g) $=$ 1 emu/g $\to $ 1 A$\cdot $m$^{2}$/kg \\
% $j$& 
% magnetic dipole \par moment& 
% 1 erg/G $=$ 1 emu \par $\to 4\pi \times  10^{-10}$ Wb$\cdot $m \\
% $J$& 
% magnetic polarization& 
% 1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 4\pi \times  10^{-4}$ T \\
% $\chi , \kappa $& 
% susceptibility& 
% 1 $\to  4\pi $ \\
% $\chi_{\rho }$& 
% mass susceptibility& 
% 1 cm$^{3}$/g $\to  4\pi \times  10^{-3}$ m$^{3}$/kg \\
% $\mu $& 
% permeability& 
% 1 $\to  4\pi \times  10^{-7}$ H/m \par $= 4\pi \times  10^{-7}$ Wb/(A$\cdot $m) \\
% $\mu_{r}$& 
% relative permeability& 
% $\mu \to \mu_{r}$ \\
% $w, W$& 
% energy density& 
% 1 erg/cm$^{3} \to  10^{-1}$ J/m$^{3}$ \\
% $N, D$& 
% demagnetizing factor& 
% 1 $\to  1/(4\pi )$ \\
% \hline
% \multicolumn{3}{p{251pt}}{Vertical lines are optional in tables. Statements that serve as captions for 
% the entire table do not need footnote letters. }\\
% \multicolumn{3}{p{251pt}}{$^{\mathrm{a}}$Gaussian units are the same as cg emu for magnetostatics; Mx 
% $=$ maxwell, G $=$ gauss, Oe $=$ oersted; Wb $=$ weber, V $=$ volt, s $=$ 
% second, T $=$ tesla, m $=$ meter, A $=$ ampere, J $=$ joule, kg $=$ 
% kilogram, H $=$ henry.}
% \end{tabular}
% \label{tab1}
% \end{table}

